Automatic Regularization for Linear MMSE Filters

In this work, we consider the problem of regularization in the design of minimum mean square error (MMSE) linear filters. Using the relationship with statistical machine learning methods, using a Bayesian approach, the regularization parameter is found from the observed signals in a simple and automatic manner. The proposed approach is illustrated in system identification and beamforming examples, where the automatic regularization is shown to yield near-optimal results.

==> Common.Files/included_packages.tex <==
\usepackage{amsmath,amssymb,amscd,latexsym,dsfont,wasysym,bbm}
%\usepackage{txfonts}  %% transforms the fonts into Times-New-Roman style
\usepackage{float}
\usepackage{color}
\usepackage{graphicx,subfigure}
\usepackage{multirow,multicol} 
\usepackage{verbatim}
\usepackage{psfrag}
\usepackage{comment}
\usepackage{makeidx}
\usepackage[]{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
%\usepackage{cite}
\usepackage{cases}
%\usepackage{amsthm}
 \usepackage{setspace}
%\usepackage[table]{xcolor}
\usepackage{pgfplots} %%%% added by LS for the errata 7.sept.2015
%\usepackage{subdepth} %%% To fix the alignment of the subscripts. It helps, but it also makes {?BICM-ID.SumExp.m1} look horrible!

==> figures/tree-nd-recursive.tex <==
\begin{tikzpicture}[level distance=2cm,
level 1/.style={sibling distance=2cm},
level 2/.style={sibling distance=2cm},
level 4/.style={sibling distance=4cm}]
\node[circle,draw]{$\bh$}
child {node[circle,draw]{$\bh^{(1)}_{l_1}$}}
child {
    node[circle,draw]{$\bg^{(1)}_{l_1}$}
    child {node[circle,draw]{$\bh^{(2)}_{l_{1},l_{2}}$}}
    child {
        node[circle,draw]{$\bg^{(2)}_{l_{1},l_{2}}$}
        child {node[circle,draw]{$\bh^{(3)}_{l_{1},l_{2},l_{3}}$}}
        child {
            node[circle,draw]{$\bg^{(N-1)}_{l_{1},\ld,l_{N-1}}$} edge from parent[dashed]
            child[solid] {node[circle,draw]{$\bh^{(N-1)}_{l_{1},\ld,p_{N-1}}$}}
            child[solid] {node[circle,draw]{$\bh^{(N)}_{l_{1},\ld,p_{N-1}}$}}
        }
    }
};
\end{tikzpicture}

==> figures/tree3d-cp.tex <==
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=2cm},
  level 2/.style={sibling distance=1.5cm}]
  \node[circle,draw]{$\bh$}
    child {node[circle,draw]{$\bh_p^{(1)}$}}
    child {node[circle,draw]{$\bh_p^{(2)}$}}
    child {node[circle,draw]{$\bh_p^{(3)}$}};
\end{tikzpicture}

==> figures/tree3d.tex <==
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=2cm},
  level 2/.style={sibling distance=2cm}]
  \node[circle,draw]{$\bh$}
    child {node[circle,draw]{$\bh^{(1)}_{l_1}$}
    }
    child {node[circle,draw]{$\bg^{(1)}_{l_1}$}
      child {node[circle,draw]{$\bh^{(2)}_{l_1 l_2}$}}
      child {node[circle,draw]{$\bh^{(3)}_{l_1 l_2}$}}
    };
\end{tikzpicture}

==> figures/tree4d-cp.tex <==
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=2cm},
  level 2/.style={sibling distance=1.5cm}]
  \node[circle,draw]{$\bh$}
    child {node[circle,draw]{$\bh_p^{(1)}$}}
    child {node[circle,draw]{$\bh_p^{(2)}$}}
    child {node[circle,draw]{$\bh_p^{(3)}$}}
    child {node[circle,draw]{$\bh_p^{(4)}$}};
\end{tikzpicture}

==> figures/tree4d-recursive.tex <==
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=2cm},
  level 2/.style={sibling distance=2cm}]
  \node[circle,draw]{$\bh$}
    child {node[circle,draw]{$\bh^{(1)}_{l_1}$}}
    child {
    node[circle,draw]{$\bg^{(1)}_{l_1}$}
    child {node[circle,draw]{$\bh^{(2)}_{l_1 l_2}$}}
    child {
    node[circle,draw]{$\bg^{(2)}_{l_1 l_2}$}
    child {node[circle,draw]{$\bh^{(3)}_{l_1 l_2 l_3}$}}
    child {node[circle,draw]{$\bh^{(4)}_{l_1 l_2 l_3}$}}
    }
    };
\end{tikzpicture}

==> figures/tree4d.tex <==
\begin{tikzpicture}[level distance=1.5cm,
  level 1/.style={sibling distance=4cm},
  level 2/.style={sibling distance=2cm}]
  \node[circle,draw]{$\bh$}
    child {node[circle,draw]{$\bh^{(1,1)}_{l_1}$}
      child {node[circle,draw]{$\bh^{(2,1)}_{l_1 l_2}$}}
      child {node[circle,draw]{$\bh^{(2,2)}_{l_1 l_2}$}}
    }
    child {node[circle,draw]{$\bh^{(1,2)}_{l_1}$}
    child {node[circle,draw]{$\bh^{(2,3)}_{l_1 l_3}$}}
      child {node[circle,draw]{$\bh^{(2,4)}_{l_1 l_3}$}}
    };
\end{tikzpicture}
